GPTNT: Benchmarking Real-Time Collaboration Between Multimodal Agents on Keep Talking And Nobody Explodes

Multimodal models are increasingly deployed to solve tasks collaboratively with humans or other artificial agents. While existing benchmarks show that they possess the fundamental capabilities, the various conditions that coincide when collaborating---time pressure, information asymmetry, and imperfect communication---have traditionally been studied in isolation. To address this gap, we introduce GPTNT, a benchmark built on the cooperative video game Keep Talking and Nobody Explodes, in which two agents must coordinate to defuse procedurally generated bomb puzzles against a live countdown. One agent has access to the bomb but not the instructions for defusing it; the other holds the instructions but cannot see or manipulate the bomb. Neither agent can succeed alone: the task requires contributions from both, and is solvable only through effective, efficient communication. We remove turn-taking proxies or simplifications, instead requiring agents to act asynchronously and communicate in real time. GPTNT is designed to expose how models collaborate versus how they perform alone: the instruction manual, the partner, or both, can optionally be withheld to surface what a model has memorised versus what it derives in the moment. We demonstrate that GPTNT poses a considerable challenge to the state-of-the-art: not one of the closed- and open-source models we test defuses a single bomb in real time, a bar that human players clear. In a range of controlled experiments, we explore where capabilities break down, identifying critical weaknesses in state tracking, efficient acting within the time budget, handling ambiguity, and error recovery. Since it runs on the real game, GPTNT benefits from procedural generation and inherits a living modding community: as models improve, the benchmark can be evolved to remain challenging, rather than being solved once and retired.

==> figures/som-creation.tex <==
\begin{figure}[tb]
\centering
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \begin{tikzpicture}
    \clip [rounded corners=5pt] (0,0) rectangle (1\textwidth, 1\textwidth);
    \node[anchor=south west, inner sep=0] at (0,0)
        {\includegraphics[width=1\textwidth]{assets/raw.png}};
    \end{tikzpicture}
    \caption{Original frame}
    \label{fig:som-original}
\end{subfigure}%
\hspace{\fill}
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \begin{tikzpicture}
    \clip [rounded corners=5pt] (0,0) rectangle (1\textwidth, 1\textwidth);
    \node[anchor=south west, inner sep=0] at (0,0)
        {\includegraphics[width=1\textwidth]{assets/segmentation.png}};
    \end{tikzpicture}
    \caption{Segmentation mask}
    \label{fig:som-segm-mask}
\end{subfigure}%
\hspace{\fill}
\begin{subfigure}[t]{0.30\textwidth}
    \centering
    \begin{tikzpicture}
    \clip [rounded corners=5pt] (0,0) rectangle (1\textwidth, 1\textwidth);
    \node[anchor=south west, inner sep=0] at (0,0)
        {\includegraphics[width=1\textwidth]{assets/som.png}};
    \end{tikzpicture}
    \caption{Image with annotations}
    \label{fig:som-final}
\end{subfigure}%
\caption{Set-of-Marks annotation inputs and outputs. The original frame (a) and segmentation mask (b) are both provided by the environment using our mod. In the segmentation mask, each interactable object is represented by a distinct colour region. Using a heuristic pipeline, we generate the annotated image (c) which combines the previous two images and provide that to the model to facilitate easier identification of interactable elements.}
\label{fig:som-creation}
\end{figure}



==> figures/som-per-module-examples.tex <==
\begin{figure}[htb]
\centering
\begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \clip [rounded corners=5pt] (0,0) rectangle (0.8\textwidth, 0.8\textwidth);
        \node[anchor=south west, inner sep=0] at (0,0)
            {\includegraphics[width=0.8\textwidth]{assets/wires_full_som.png}};
    \end{tikzpicture}
    \caption{Wires}
    \label{fig:sub-wires}
\end{subfigure}%
% \hspace{\fill}
\begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \clip [rounded corners=5pt] (0,0) rectangle (0.8\textwidth, 0.8\textwidth);
        \node[anchor=south west, inner sep=0] at (0,0)
            {\includegraphics[width=0.8\textwidth]{assets/simon_som.png}};
    \end{tikzpicture}
    \caption{Simon Says}
    \label{fig:simon_som}
\end{subfigure}%
% \hspace{\fill}
\begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \clip [rounded corners=5pt] (0,0) rectangle (0.8\textwidth, 0.8\textwidth);
        \node[anchor=south west, inner sep=0] at (0,0)
            {\includegraphics[width=0.8\textwidth]{assets/comp_wires_som.png}};
    \end{tikzpicture}
    \caption{Complicated\\Wires}
    \label{fig:comp-wires-som}
\end{subfigure}%
% \hspace{\fill}
\begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \clip [rounded corners=5pt] (0,0) rectangle (0.8\textwidth, 0.8\textwidth);
        \node[anchor=south west, inner sep=0] at (0,0)
            {\includegraphics[width=0.8\textwidth]{assets/keypad_som.png}};
    \end{tikzpicture}
    \caption{Keypad}
    \label{fig:keypad-som}
\end{subfigure}%
% \hspace{\fill}
\begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \clip [rounded corners=5pt] (0,0) rectangle (0.8\textwidth, 0.8\textwidth);
        \node[anchor=south west, inner sep=0] at (0,0)
            {\includegraphics[width=0.8\textwidth]{assets/whos_on_first_som.png}};
    \end{tikzpicture}
    \caption{Who's On First}
    \label{fig:whosonfirst-som}
\end{subfigure}
\caption{Examples of set-of-marks annotations applied to different bomb modules where colour is important to distinguish between elements.}
\label{fig:som-per-module-example}
\end{figure}




==> tables/results/E1-behaviour-pct-w-average.tex <==
% \begin{table}[tbh]\centering\footnotesize\renewcommand{\arraystretch}{1.4}
% \begin{threeparttable}
% \caption{Proportion of steps a player chose to wait, navigate (Nav), interact with objects (Int), or send a message (Msg) by game outcome.}
% \label{tab:e1-behavior}
% \begin{tabular}{@{}p{1.0mm} l c c c c c c c c c c c c @{}}\toprule
%  & &  \multicolumn{4}{c}{\success*} & \multicolumn{4}{c}{\strikeout*} & \multicolumn{4}{c}{\timeout*}\\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
% & & {\scriptsize Wait} & {\scriptsize Msg} & {\scriptsize Nav} & {\scriptsize Int} & {\scriptsize Wait} & {\scriptsize Msg} & {\scriptsize Nav} & {\scriptsize Int} & {\scriptsize Wait} & {\scriptsize Msg} & {\scriptsize Nav} & {\scriptsize Int}\\ \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\textls[25]{Defuser}}}} & \claude*~Sonnet 4.6 & 3.9 & 22.0 & 26.9 & 47.3 & 4.8 & 22.9 & 24.0 & 48.3 & 8.1 & 13.0 & 50.1 & 28.8\\
%   & \gemini*~Gemini 3 Flash & 2.5 & 30.9 & 21.7 & 44.8 & 1.3 & 33.7 & 18.2 & 46.7 & 0.9 & 8.6 & 71.1 & 19.5\\
%   & \openai*~GPT-5.2 & 5.0 & 31.7 & 15.4 & 47.9 & 4.8 & 39.2 & 12.2 & 43.8 & 9.0 & 31.6 & 38.8 & 20.6\\
%   & \internvl*~InternVL 3.5 (38B) & 15.3 & 42.8 & 4.8 & 37.1 & 9.2 & 43.6 & 4.9 & 42.3 & 34.8 & 31.7 & 17.6 & 16.0\\
%   & \qwen*~Qwen3.5 (27B) & 5.6 & 29.5 & 24.6 & 40.3 & 4.7 & 35.6 & 17.7 & 42.0 & 15.0 & 20.5 & 47.4 & 17.1\\
% \midrule[0.1ex]
%   & \textit{Average} & 6.5 & 31.4 & 18.7 & 43.5 & 5.0 & 35.0 & 15.4 & 44.6 & 13.6 & 21.1 & 45.0 & 20.4\\
% \midrule[0.1ex]
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\textls[25]{Expert}}}} & \claude*~Sonnet 4.6 & 60.4 & 39.6 & \color{black!40}0.0 & \color{black!40}0.0 & 60.2 & 39.8 & \color{black!40}0.0 & \color{black!40}0.0 & 74.0 & 26.0 & \color{black!40}0.0 & \color{black!40}0.0\\
%   & \gemini*~Gemini 3 Flash & 49.1 & 50.9 & \color{black!40}0.0 & \color{black!40}0.0 & 48.9 & 51.1 & \color{black!40}0.0 & \color{black!40}0.0 & 60.4 & 39.6 & \color{black!40}0.0 & \color{black!40}0.0\\
%   & \openai*~GPT-5.2 & 61.2 & 38.8 & \color{black!40}0.0 & \color{black!40}0.0 & 59.4 & 40.6 & \color{black!40}0.0 & \color{black!40}0.0 & 72.9 & 27.1 & \color{black!40}0.0 & \color{black!40}0.0\\
%   & \internvl*~InternVL 3.5 (38B) & 65.9 & 34.1 & \color{black!40}0.0 & \color{black!40}0.0 & 60.9 & 39.1 & \color{black!40}0.0 & \color{black!40}0.0 & 75.0 & 25.0 & \color{black!40}0.0 & \color{black!40}0.0\\
%   & \qwen*~Qwen3.5 (27B) & 61.0 & 39.0 & \color{black!40}0.0 & \color{black!40}0.0 & 57.1 & 42.9 & \color{black!40}0.0 & \color{black!40}0.0 & 68.2 & 31.8 & \color{black!40}0.0 & \color{black!40}0.0\\
% \midrule[0.1ex]
%   & \textit{Average} & 59.5 & 40.5 & \color{black!40}0.0 & \color{black!40}0.0 & 57.3 & 42.7 & \color{black!40}0.0 & \color{black!40}0.0 & 70.1 & 29.9 & \color{black!40}0.0 & \color{black!40}0.0\\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}[flushleft]
%     \footnotesize
%     \item \success* Solved. \strikeout* Strikeout. \timeout* Timeout.
% \end{tablenotes}
% \end{threeparttable}\end{table}

\begin{table}[tbh]\centering\footnotesize\renewcommand{\arraystretch}{1.4}
\begin{threeparttable}
\caption{Distribution of action types (\% of game steps) by model, role and game outcome played by all possible model pairings on single-module missions in \textit{synchronous} mode. Both players can either wait or send a message (Msg). The Defuser can additionally navigate (Nav) or interact with objects (Int).}
\label{tab:e1-behavior}
\begin{tabular}{@{}p{1.0mm} l c c c c c c c c c c c c @{}}\toprule
 & &  \multicolumn{4}{c}{\success* Solved} & \multicolumn{4}{c}{\strikeout* Strikeout} & \multicolumn{4}{c}{\timeout* Timeout}\\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
& & {\scriptsize Wait} & {\scriptsize Msg} & {\scriptsize Nav} & {\scriptsize Int} & {\scriptsize Wait} & {\scriptsize Msg} & {\scriptsize Nav} & {\scriptsize Int} & {\scriptsize Wait} & {\scriptsize Msg} & {\scriptsize Nav} & {\scriptsize Int}\\ \midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\textls[25]{Defuser}}}} & \claude*~Sonnet 4.6 & 3.9 & 22.0 & 26.9 & 47.3 & 4.8 & 22.9 & 24.0 & 48.3 & 8.1 & 13.0 & 50.1 & 28.8\\
  & \gemini*~Gemini 3 Flash & 2.5 & 30.9 & 21.7 & 44.8 & 1.3 & 33.7 & 18.2 & 46.7 & 0.9 & 8.6 & 71.1 & 19.5\\
  & \openai*~GPT-5.2 & 5.0 & 31.8 & 15.3 & 47.8 & 4.8 & 39.5 & 12.2 & 43.6 & 9.0 & 31.7 & 38.8 & 20.5\\
  & \internvl*~InternVL 3.5 (38B) & 15.3 & 42.8 & 4.8 & 37.1 & 9.2 & 43.6 & 4.9 & 42.3 & 34.8 & 31.7 & 17.6 & 16.0\\
  & \qwen*~Qwen3.5 (27B) & 5.6 & 29.5 & 24.6 & 40.3 & 4.7 & 35.6 & 17.7 & 42.0 & 15.0 & 20.5 & 47.4 & 17.1\\
\midrule[0.1ex]
  & \textit{Average} & 6.5 & 31.4 & 18.7 & 43.5 & 4.9 & 35.1 & 15.4 & 44.6 & 13.6 & 21.1 & 45.0 & 20.4\\
\midrule[0.1ex]
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{\textls[25]{Expert}}}} & \claude*~Sonnet 4.6 & 60.4 & 39.6 & \color{black!40}0.0 & \color{black!40}0.0 & 60.2 & 39.8 & \color{black!40}0.0 & \color{black!40}0.0 & 74.0 & 26.0 & \color{black!40}0.0 & \color{black!40}0.0\\
  & \gemini*~Gemini 3 Flash & 49.1 & 50.9 & \color{black!40}0.0 & \color{black!40}0.0 & 48.9 & 51.1 & \color{black!40}0.0 & \color{black!40}0.0 & 60.4 & 39.6 & \color{black!40}0.0 & \color{black!40}0.0\\
  & \openai*~GPT-5.2 & 61.1 & 38.9 & \color{black!40}0.0 & \color{black!40}0.0 & 59.3 & 40.7 & \color{black!40}0.0 & \color{black!40}0.0 & 72.7 & 27.3 & \color{black!40}0.0 & \color{black!40}0.0\\
  & \internvl*~InternVL 3.5 (38B) & 65.9 & 34.1 & \color{black!40}0.0 & \color{black!40}0.0 & 60.9 & 39.1 & \color{black!40}0.0 & \color{black!40}0.0 & 75.0 & 25.0 & \color{black!40}0.0 & \color{black!40}0.0\\
  & \qwen*~Qwen3.5 (27B) & 61.0 & 39.0 & \color{black!40}0.0 & \color{black!40}0.0 & 57.1 & 42.9 & \color{black!40}0.0 & \color{black!40}0.0 & 68.2 & 31.8 & \color{black!40}0.0 & \color{black!40}0.0\\
\midrule[0.1ex]
  & \textit{Average} & 59.5 & 40.5 & \color{black!40}0.0 & \color{black!40}0.0 & 57.3 & 42.7 & \color{black!40}0.0 & \color{black!40}0.0 & 70.1 & 29.9 & \color{black!40}0.0 & \color{black!40}0.0\\
\bottomrule
\end{tabular}
\end{threeparttable}\end{table}

==> tables/results/table_e5_outcomes.tex <==
% \begin{table}[tbh]\centering\footnotesize\renewcommand{\arraystretch}{1.4}
% \begin{threeparttable}
% \caption{Game outcomes details for self-play across ten distinct missions in synchronous mode. In the synchronous setting, we stop the game clock while models take turns generating. Each mission is attempted once (pass@1).}
% \label{tab:e5-stats}
% \setlength{\tabcolsep}{4pt}
% \sisetup{table-format=2.1}
% \begin{tabular}{@{}l SSSSSS[table-format=3.1] S @{}}\toprule
% Model & {\makecell{\% Modules\\Solved}} & {\makecell{\% Failed\\Strikeout}} & {\makecell{Strikeout @\\\% Game}} & {\makecell{\% Failed\\Timeout}} & {\makecell{Timeout\\0 Strikes}} & {\makecell{Timeout\\1 Strike}} & {\makecell{Timeout\\2 Strikes}} \\ \midrule
% \claude*~Sonnet 4.6 & 30.0 & 66.7 & 25.3 & 33.3 & 33.3 & \color{black!40}0.0 & 66.7\\
% \gemini*~Gemini 3 Flash & 15.8 & 40.0 & 30.7 & 60.0 & 50.0 & 33.3 & 16.7\\
% \openai*~GPT-5.2 & 22.5 & 77.8 & 52.4 & 22.2 & \color{black!40}0.0 & 100.0 & \color{black!40}0.0\\
% \internvl*~InternVL 3.5 (38B) & 11.7 & 30.0 & 20.4 & 70.0 & 28.6 & 14.3 & 57.1\\
% \qwen*~Qwen3.5 (27B) & 11.7 & 40.0 & 28.6 & 60.0 & 66.7 & 33.3 & \color{black!40}0.0\\
% \midrule
% \textit{Average} & 18.3 & 50.9 & 31.5 & 49.1 & 35.7 & 36.2 & 28.1\\
% \bottomrule
% \end{tabular}
% \end{threeparttable}\end{table}

\begin{table}[tbh]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.4}
\begin{threeparttable}
\caption{Self-play game outcomes across ten distinct missions in \textit{synchronous} mode, where the game \textit{is paused} while models generate. We examine module completion, strike distribution at timeout, and strikeout timing. Each mission is attempted once (pass@1).}
\label{tab:e5-stats}
\sisetup{table-format=2.1}
\begin{tabular}{@{}l S S S S[table-format=3.1] S S S @{}}
\toprule
 &  & \multicolumn{4}{c}{\timeout* Timeout} & \multicolumn{2}{c}{\strikeout* Strikeout} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-8}
 & {\makecell{\% Modules\\Solved}}
 & {\makecell{\% of\\Failures}}
 & {0 Strikes}
 & {1 Strike}
 & {2 Strikes}
 & {\makecell{\% of\\Failures}}
 & {\makecell{Time\\Elapsed (\%)}} \\
\midrule
\claude*~Sonnet 4.6           & 30.0 & 33.3 & 33.3 & \color{black!40}0.0  & 66.7 & 66.7 & 25.3 \\
\gemini*~Gemini 3 Flash       & 15.8 & 60.0 & 50.0 & 33.3                 & 16.7 & 40.0 & 30.7 \\
\openai*~GPT-5.2              & 22.5 & 22.2 & \color{black!40}0.0 & 100.0 & \color{black!40}0.0 & 77.8 & 52.4 \\
\internvl*~InternVL 3.5 (38B) & 11.7 & 70.0 & 28.6 & 14.3                 & 57.1 & 30.0 & 20.4 \\
\qwen*~Qwen3.5 (27B)          & 11.7 & 60.0 & 66.7 & 33.3                 & \color{black!40}0.0 & 40.0 & 28.6 \\
\midrule
\textit{Average}              & 18.3 & 49.1 & 35.7 & 36.2                 & 28.1 & 50.9 & 31.5 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}

==> tables/results/table_e7_outcomes.tex <==
% \begin{table}[tbh]\centering\footnotesize\renewcommand{\arraystretch}{1.4}
% \begin{threeparttable}
% \caption{Game outcome details for self-play across ten distinct missions in asynchronous mode. In the asynchronous setting, we do not stop the game clock while models are generating. Each mission is attempted once (pass@1).}
% \label{tab:e7-stats}
% \sisetup{table-format=2.1}
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{@{}l SSSSSSS @{}}\toprule
% Model & {\makecell{\% Modules\\Solved}} & {\makecell{\% Failed\\Strikeout}} & {\makecell{Strikeout @\\\% Game}} & {\makecell{\% Failed\\Timeout}} & {\makecell{Timeout\\0 Strikes}} & {\makecell{Timeout\\1 Strike}} & {\makecell{Timeout\\2 Strikes}} \\ \midrule
% \claude*~Sonnet 4.6 & 15.8 & 60.0 & 65.0 & 40.0 & 25.0 & 25.0 & 50.0\\
% \gemini*~Gemini 3 Flash & 10.0 & 50.0 & 47.0 & 50.0 & 80.0 & \color{black!40}0.0 & 20.0\\
% \openai*~GPT-5.2 & 11.7 & 10.0 & 65.0 & 90.0 & 33.3 & 33.3 & 33.3\\
% \internvl*~InternVL 3.5 (38B) & 3.3 & 30.0 & 18.3 & 70.0 & 57.1 & 14.3 & 28.6\\
% \qwen*~Qwen3.5 (27B) & 6.7 & 20.0 & 43.1 & 80.0 & 75.0 & 25.0 & \color{black!40}0.0\\
% \midrule
% \textit{Average} & 9.5 & 34.0 & 47.7 & 66.0 & 54.1 & 19.5 & 26.4\\
% \bottomrule
% \end{tabular}
% \end{threeparttable}\end{table}

\begin{table}[tbh]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.4}
\begin{threeparttable}
\caption{Self-play game outcomes across ten distinct missions in asynchronous mode, where the game is \textit{not paused} while models generate. We examine module completion, strike distribution at timeout, and strikeout timing. Each mission is attempted once (pass@1).}
\label{tab:e7-stats}
\sisetup{table-format=2.1}
% \setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}l S S S S S S S @{}}
\toprule
 & {} & \multicolumn{4}{c}{\timeout* Timeout} & \multicolumn{2}{c}{\strikeout* Strikeout} \\
\cmidrule(lr){3-6}\cmidrule(l){7-8}
 & {\makecell{\% Modules\\Solved}}
 & {\makecell{\% of\\Failures}}
 & {0 Strikes}
 & {1 Strike}
 & {2 Strikes}
 & {\makecell{\% of\\Failures}}
 & {\makecell{Time\\Elapsed (\%)}} \\
\midrule
\claude*~Sonnet 4.6           & 15.8 & 40.0 & 25.0 & 25.0 & 50.0 & 60.0 & 65.0 \\
\gemini*~Gemini 3 Flash       & 10.0 & 50.0 & 80.0 & \color{black!40}0.0 & 20.0 & 50.0 & 47.0 \\
\openai*~GPT-5.2              & 11.7 & 90.0 & 33.3 & 33.3 & 33.3 & 10.0 & 65.0 \\
\internvl*~InternVL 3.5 (38B) & 3.3  & 70.0 & 57.1 & 14.3 & 28.6 & 30.0 & 18.3 \\
\qwen*~Qwen3.5 (27B)          & 6.7  & 80.0 & 75.0 & 25.0 & \color{black!40}0.0 & 20.0 & 43.1 \\
\midrule
\textit{Average}              & 9.5  & 66.0 & 54.1 & 19.5 & 26.4 & 34.0 & 47.7 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}

==> tables/statics/statics-localisation-module-breakdown-w-average.tex <==
\begin{table}[tbh]\centering\footnotesize\renewcommand{\arraystretch}{1.4}
\begin{threeparttable}
\sisetup{table-format=2.1}
\caption{Accuracy (\%) on Simulator Localisation tasks comparing selecting the correct set-of-marks style location marker with predicting a valid coordinate for actions.}
\label{tab:localization-coordinates-vs-som}
\begin{tabular}{@{}p{1.0mm} l *{11}{S} S @{}}\toprule
 & &  {\wires*} & {\button*} & {\keypad*} & {\simonsays*} & {\whosonfirst*} & {\memory*} & {\maze*} & {\morsecode*} & {\complicatedwires*} & {\wiresequence*} & {\passwords*} & {\textit{Avg.}}\\ \midrule
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{\textls[25]{Set-of-Marks}}}}} & \claude*~Sonnet 4.6 & 64.3 & \Uline{100.0} & 71.7 & \Uline{100.0} & 77.8 & 95.5 & \Uline{100.0} & \Uline{100.0} & \Uline{74.0} & 60.9 & 76.5 & 80.6 \\
 & \gemini*~Gemini 3 Flash & 64.3 & \Uline{100.0} & \Uline{98.1} & \Uline{100.0} & 53.7 & \Uline{100.0} & \Uline{100.0} & \Uline{100.0} & \Uline{74.0} & \Uline{69.6} & \Uline{97.1} & \Uline{83.9} \\
 & \openai*~GPT-5.2 & \Uline{71.4} & \Uline{100.0} & 81.1 & \Uline{100.0} & 68.5 & 95.5 & \Uline{100.0} & 96.9 & 72.0 & 67.4 & 64.7 & 80.4 \\
 & \internvl*~InternVL 3.5 (38B) & 50.0 & 95.5 & 71.7 & 66.7 & 22.2 & 18.2 & \Uline{100.0} & 65.6 & 58.0 & 37.0 & 23.5 & 53.7 \\
 & \qwen*~Qwen3.5 (27B) & 64.3 & \Uline{100.0} & 73.6 & \Uline{100.0} & 70.4 & \Uline{100.0} & \Uline{100.0} & 96.9 & 64.0 & 58.7 & 58.8 & 76.8 \\
\cmidrule[0.1ex](l){2-14}
 & \textit{Average} & 62.9 & 99.1 & 79.2 & 93.3 & 58.5 & 81.8 & 100.0 & 91.9 & 68.4 & 58.7 & 64.1 & 75.1 \\
\midrule
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{\textls[25]{Coordinates}}}}} & \claude*~Sonnet 4.6 & 17.9 & 90.9 & 73.6 & 90.5 & 87.0 & 40.9 & 11.4 & 53.1 & 8.0 & 13.0 & 20.6 & 44.6 \\
 & \gemini*~Gemini 3 Flash & 10.7 & 90.9 & 92.5 & 90.5 & \Uline{96.3} & 86.4 & 68.6 & 84.4 & 30.0 & 37.0 & 82.4 & 68.8 \\
 & \openai*~GPT-5.2 & 3.6 & 27.3 & 1.9 & 4.8 & 1.9 & 4.5 & 2.9 & \color{black!40}0.0 & 4.0 & 2.2 & \color{black!40}0.0 & 4.5 \\
 & \internvl*~InternVL 3.5 (38B) & 7.1 & 90.9 & 52.9 & 38.1 & 52.8 & \color{black!40}0.0 & \color{black!40}0.0 & 21.9 & 2.0 & 6.5 & 11.8 & 29.6 \\
 & \qwen*~Qwen3.5 (27B) & 23.1 & \Uline{100.0} & 65.1 & 78.9 & 88.5 & 72.7 & 12.5 & 70.0 & 11.6 & 31.0 & 6.2 & 49.4 \\
\cmidrule[0.1ex](l){2-14}
 & \textit{Average} & 12.5 & 80.0 & 57.2 & 60.6 & 65.3 & 40.9 & 19.1 & 45.9 & 11.1 & 17.9 & 24.2 & 39.4 \\
\bottomrule
\end{tabular}
\end{threeparttable}\end{table}
